Strategy Complexity of Point Payoff, Mean Payoff and Total Payoff Objectives in Countable MDPs

We study countably infinite Markov decision processes (MDPs) with real-valued transition rewards. Every infinite run induces the following sequences of payoffs: 1. Point payoff (the sequence of directly seen transition rewards), 2. Mean payoff (the sequence of the sums of all rewards so far, divided by the number of steps), and 3. Total payoff (the sequence of the sums of all rewards so far). For each payoff type, the objective is to maximize the probability that the $\liminf$ is non-negative. We establish the complete picture of the strategy complexity of these objectives, i.e., how much memory is necessary and sufficient for $\varepsilon$-optimal (resp. optimal) strategies. Some cases can be won with memoryless deterministic strategies, while others require a step counter, a reward counter, or both.

==> Figures/summarytable.tex <==
\begin{center}
\begin{tabular}{ |p{3.5cm}|p{3.5cm}||p{3.5cm}|p{3.5cm}|  }
 \hline
 \multicolumn{2}{|c||}{Liminf TP} & \multicolumn{2}{|c|}{Liminf MP} \\
 \hline
 Lower Bound & Upper Bound & Lower Bound & Upper Bound\\
 \hline
 $\eps$-optimal/almost-sure   & $\eps$-optimal    & $\eps$-optimal & Almost-sure/Optimal\\
 Reward Counter &   Reward Counter  &  Markov?  & Acyclic $\to$ MD \\
 Markov & Acyclic $\to$ MD & Reward Counter? & General $\to$ Markov  \\
  & Finite Branching $\to$ MD & PFA? &  $\eps$-optimal \\
  & General $\to$ Markov  & Infinite Memory in some form & Markov + Reward counter + 1-bit \\
 \hline
\end{tabular}
\end{center}

==> liminf-upper.tex <==
We establish upper bounds on the strategy complexity
of $\liminf$ threshold objectives for mean payoff, total payoff and point payoff.
It is noteworthy that once the reward structure of an MDP has been encoded into the states,
then these threshold objectives take on a qualitative flavor not
dissimilar to Safety or co-B\"{u}chi (cf.~\cite{KMSW2017}).
Indeed, if the transition rewards are restricted to integer values,
then $\liminftpobj$ boils down to eventually avoiding all transitions with
negative reward (since negative rewards would be $\le -1$).
This is a co-B\"{u}chi objective.
However, if the rewards are not restricted to integers, then the picture is not so simple.





















% \begin{remark}
% While $\eps$-optimal strategies for mean payoff and total payoff
% (in infinitely branching MDPs) have the same memory requirements, the step counter and the reward counter do not arise in the same way.
% Both the step counter and reward counter used in $\eps$-optimal strategies for mean payoff  arise from the construction of $A(\mdp)$. However, in the case for total payoff, only the reward counter arises from the construction of $R(\mdp)$. The step counter on the other hand arises from the Markov strategy needed for point payoff in $R(\mdp)$.
% \end{remark}



